Distributing many points on spheres: minimal energy and designs

This survey discusses recent developments in the context of spherical designs and minimal energy point configurations on spheres. The recent solution of the long standing problem of the existence of spherical $t$-designs on $\mathbb{S}^d$ with $\mathcal{O}(t^d)$ number of points by A. Bondarenko, D. Radchenko, and M. Viazovska attracted new interest to this subject. Secondly, D. P. Hardin and E. B. Saff proved that point sets minimising the discrete Riesz energy on $\mathbb{S}^d$ in the hypersingular case are asymptotically uniformly distributed. Both results are of great relevance to the problem of describing the quality of point distributions on $\mathbb{S}^d$, as well as finding point sets, which exhibit good distribution behaviour with respect to various quality measures.

==> Energy.tex <==
\section{Energy}\label{sec:energy}


\subsection{Minimal energy in applications}
\label{sec:minim-energy-appl}

A surprising number of diverse applications can be formulated as a
discrete or continuous minimal energy problem (or a mixture of both). In the
discrete case this means to find a collection of $N$ points in a subset $A$ of
$\R^p$, $p \geq 1$, that minimise a \emph{discrete $\KERNEL$-energy functional}
\begin{equation*}
E_{\KERNEL,\extFIELD}(\PT{x}_1,\dots,\PT{x}_N)\DEF 
\mathop{\sum_{i = 1}^N \sum_{j = 1}^N}_{i \neq j}\Big[\KERNEL(\PT{x}_i,\PT{x}_j) 
+ \extFIELD( \PT{x}_i ) + \extFIELD( \PT{x}_j ) \Big]
\end{equation*}
incorporating an \emph{external field} $\extFIELD$ (which is often taken to be
zero), among all $N$-point tuples from $A^N$. The diagonal (self-interaction)
terms are removed to allow singular kernels~$\KERNEL$. Evidently, further
requirements on the set~$A$, the kernel $\KERNEL$ and the external field
$\extFIELD$ are needed to ensure existence of a solution. A suitable
$\extFIELD$ compatible with $\KERNEL$ prevents points from escaping to infinity
and thus introduces soft boundaries (allowing even $A = \R^p$) whereas by
restricting the points to a finite set, a fractal, a torus or a sphere of
Hausdorff dimension $d \leq p$, fractal or topological aspects enter the
picture.
%
A standard assumption is that $\KERNEL$ is symmetric and lower semi-continuous
on $A \times A$ and that $\extFIELD$ is also lower semi-continuous on $A$. This
will (roughly speaking) guarantee that the \emph{minimal $\KERNEL$-energy
  problem with external field $\extFIELD$} has a solution when solved for an infinite
compact set $A$; i.e.,
\begin{equation*}
\mathcal{E}_{\KERNEL,\extFIELD}(A;N)\DEF 
\inf\Big\{ E_{\KERNEL,\extFIELD}(\PT{x}_1,\dots,\PT{x}_N ):\PT{x}_1,\dots,\PT{x}_N\in A
\Big\} = E_{\KERNEL,\extFIELD}(\PT{x}_1^*,\dots,\PT{x}_N^*)
\end{equation*}
for an \emph{$N$-point minimal $\KERNEL$-energy configuration $X_N^* = \{
  \PT{x}_1^*, \dots, \PT{x}_N^* \}$ associated with $\extFIELD$}.
%
Furthermore, the quantities $N ( N - 1 ) / \mathcal{E}_{\KERNEL,\extFIELD}( A; N )$
form a non-increasing sequence that is bounded from below by
semi-continuity. Thus the limit exists and it discriminates between two types
of sets $A$ depending on whether or not this limit vanishes. This gives rise to
two different regimes characterised by a complete change in the nature of the
minimisation problem with regard to properties of the solution and methods that
are used to study it.
%
In the field-free setting ($\extFIELD \equiv 0$), the normalised \emph{discrete
  minimal $N$-point energy of $A$}, given by $\mathcal{E}_{\KERNEL,0}( A; N ) /
[ N ( N - 1 ) ]$, is also known as the $N$-th diameter of $A$. The limit in the
extended sense (as $N \to \infty$) is called the \emph{transfinite diameter of
  $A$}.

% 
% Sets $A$ with non-vanishing limit 
% 
% 
% the ``potential theoretic regime'' continuous or singular setting (for which
% a ``potential theory'' can be formulated) and the hypersingular setting (when
% central potential theoretic concepts fail to work).
%
% The vanishing and non-vanishing of the limit for a set $A$ is linked to the
% continuous, weakly singular or hypersingular nature of $\KERNEL$ (and
% $\extFIELD$)
%
%  are sets $A$ for which this sequence has non-zero limit.
%
A fundamental question concerns the ``limit distribution'' (if such exists) of
a sequence $(X_N^*)$ of minimal energy configurations $X_N^*$ on $A$ as $N \to
\infty$; i.e., is there a (unique) Borel probability measure $\mu_A^*$
supported on $A$ that is the weak limit of the sequence formed by the discrete
equal weight distribution supported on $X_N^*$,
\begin{equation*}
\mu_{X_N^*} \DEF \frac{1}{N} \sum_{j = 1}^N \delta_{\PT{x}}.
\end{equation*}
% of discrete equal weight distribution supported on $X_N^*$.
% 
% Each configuration $X_N^*$ in a sequence of minimal energy configurations
% defines a discrete equal weight distribution supported on $X_N^*$,
% \begin{equation*}
% \mu_{X_N^*} \DEF \frac{1}{N} \sum_{j = 1}^N \delta_{\PT{x}}.
% \end{equation*}
% A fundamental question concerns its `limit distribution'' (if such exists);
% i.e., the existence (and uniqueness) of a Borel probability measure $\mu_A$
% supported on $A$ that is the weak limit of the sequence $(\mu_{X_N^*})$.
% \begin{equation*}
% \lim_{N \to \infty} 
% \end{equation*}
% 
% Its ``limit distribution'' (if such exists) is dubbed the ``limit
% distribution'' of the minimal $\KERNEL$-energy points associated with
% $\extFIELD$.

Let $\mathcal{M}( A )$ denote the collection of Borel probability measures
supported on $A$.
%
The analogue continuous energy problem concerns the finding of a measure
supported on $A$ that minimises the \emph{weighted $\KERNEL$-energy associated
  with $\extFIELD$},
\begin{equation*}
\mathcal{I}_{\KERNEL, \extFIELD}( \mu ) \DEF \mathcal{I}_{\KERNEL}( \mu ) + 2
\int_A \extFIELD( \PT{x} ) \, \dd \sigma_d( \PT{x} ),  
\end{equation*}
which is defined by means of the \emph{$\KERNEL$-energy of the measure $\mu$ on
  $A$},
\begin{equation*}
\mathcal{I}_{\KERNEL}( \mu ) \DEF \int_A \int_A \KERNEL( \PT{x}, \PT{y} ) \, 
\dd \mu( \PT{x} ) \dd \mu( \PT{y} ),
\end{equation*}
among all Borel probability measures supported on $A$. A minimising measure
${\mu_{\KERNEL,\extFIELD; A} \in \mathcal{M}( A )}$ with
\begin{equation*}
\mathcal{I}_{\KERNEL, \extFIELD}( \mu_{\KERNEL,\extFIELD; A} ) = 
W_{\KERNEL, \extFIELD}( A ) \DEF 
\inf\Big\{ \mathcal{I}_{\KERNEL, \extFIELD}( \mu ) \  \Big| \  
\mu \in \mathcal{M}( A ) \Big\},
\end{equation*}
is called a \emph{$\KERNEL$-extremal (or positive equilibrium) measure on $A$
  associated with $\extFIELD$}. In the field free setting $\extFIELD \equiv 0$,
a minimising measure $\mu_{K;A}$ is called \emph{$\KERNEL$-equilibrium measure
  on $A$}. In this case, the $\KERNEL$-energy $\mathcal{I}_{\KERNEL}( \mu_{K;A}
)$ is equal to the \emph{Wiener energy of $A$},
\begin{equation*}
W_{\KERNEL}( A ) \DEF \inf\Big\{ \mathcal{I}_{\KERNEL}( \mu ) \  \Big| \  
\mu \in \mathcal{M}( A ) \Big\}.
\end{equation*}
A fundamental question concerns the relation between the Wiener energy of $A$,
the transfinite diameter of $A$ and the Chebyshev constant of $A$ which is the
limit as $N \to \infty$ of the $N$-th Chebyshev constant of $A$ defined as
\begin{equation*}
M_N( A ) \DEF \sup_{\PT{x}_1, \dots, \PT{x}_N \in A} \inf_{\PT{x} \in A} 
\frac{1}{N} \sum_{j=1}^N \KERNEL( \PT{x}, \PT{x}_j );
\end{equation*}
see~\cite{FaNa2008} and references cited therein for further details.


% A Borel probability measure $\mu_{\KERNEL,\extFIELD}$ supported on $A$ that 


% The continuous, weakly singular or hypersingular nature of $\KERNEL$ can
% completely change the character of the minimization problem.
% 
% 
% A satisfactory treatment of the 

 

Next, we discuss applications which make use of the minimal energy problem. 

\begin{description}
\item[The Thomson problem and its generalisation.] A classical problem in
  electrostatics is to find the distribution of $N$ unit point charges on a
  conductor in the most-stable equilibrium (the charges interact according to
  the Coulomb potential $1/r$, where $r$ is the Euclidean distance between two
  interacting charges). This leads to a minimisation problem for the potential
  energy of the discrete charge system named after J.~J.~Thomson who posed it
  for the sphere~\cite{thomson:1904}.
%
  A generalisation of Thomson problem using general laws of interactions (Riesz
  $s$-potential $1/r^s$) include multi-electron bubbles and arrangements of
  protein subunits which form the shells (or capsid) of spherical viruses; see
  \cite{Bowick_Cacciuto_Nelson+2002:crystalline_order_sphere}
  (cf.~\cite{Bowick_Giomi2009}) for a discussion.
%

For small number of points numerical optimisation can be used to find minimal
Riesz $s$-energy configurations. As observed in \cite{MeKnSm1977}, for each $N$
there may be one or more ``basic configuration'' which compete for smallest
energy as $s$ grows from $1$ to large values. For example, no configuration of
five points can be optimal for all values of $s$
(cf.~\cite{Cohn_Kumar2007:universally_optimal_sphere}).
% for the five point
% problem on $\mathbb{S}^2$ it is clear that $5$ points cannot be universally
% optimal (cf.~\cite{Cohn_Kumar2007:universally_optimal_sphere}).
In fact, there
are two basic configuration (double pyramid and quadratic pyramid) which
compete. According to the numerical results for $−2 \leq s \leq
15.048077392\dots$ the regular triangular bi-pyramid is the putative
energy-minimising configuration whereas for higher values of $s$ it seems to be
the square pyramid (with adjusted height); see also \cite{NeBrKie2013} for a
finer analysis. In the last paper monotonicity properties of the second
discrete derivative were considered which lead to new putative low-energy
configurations in two cases.

%
\item[Half-toning.] Loosely speaking, half-toning is some way of creating an
  illusion of a grey-value image by appropriately distributing black dots. (One
  can variate from this by having only a limited number of colours available.)
  In \cite{GrPoSt2012} the authors show how the process of half-toning can be
  seen as a numerical integration process with the aim to minimise a worst-case
  error or how it can be interpreted as an external field problem where the
  picture drives the external field which guides the interacting points; see
  also \cite{TeStGw2011}.
%
\item[Maximising Determinants.] I.~Sloan and
  R.~S.~Womersley~\cite{Sloan_Womersley2004:extremal_sphere} considered points
  that maximise a Vandermonde-type determinant that appears in the polynomial
  Lagrange interpolation formula. See
  also~\cite{Marzo_Ortega-Cerda2010:equidistribution_fekete}.


\item[Diffusion on a sphere with localised traps.] As an application in
  cellular signal transport the authors of \cite{CoStWa2009} calculate the
  principal eigenvalue for the Laplacian on the unit sphere in the presence of
  $N$ traps on the surface of the sphere of asymptotically small radii. The
  positions of the traps are chosen to minimise the discrete logarithmic energy
  (cf. Section~\ref{sec:cont-minim-energy}).

% \item[Polarization.] 


\end{description}

% Abstract Fekete points are the points that maximize a Vandermonde-type
% determi- nant that appears in the polynomial Lagrange interpolation
% formula. They are well- suited points for interpolation formulas and
% numerical integration. We prove the
% 

% \subsubsection*{The Thomson problem and its generalization} 



% Numerical experiments (see~\cite{MeKnSm1977}) for up to $16$ points and $s
% \in [1,400]$ suggest that as $s$ changes



% \cite{Grabner2014:point_minimal_energy}


% Minimal energy points are used to discretize manifolds
% (\cite{Hardin_Saff2004:discretizing_manifolds}),

% \MARKED{Red}{\centerline{\Large \bf [ \dots introductory paragraph \dots ]}}




\subsection{The discrete and continuous minimal logarithmic 
and Riesz energy problem}
\label{sec:cont-minim-energy}

The discrete logarithmic energy problem on $\mathbb{S}^d$ is concerned with the
properties of $N$-point configurations $\{ \PT{x}_1^*, \dots, \PT{x}_N^* \}
\subset \mathbb{S}^d$ that maximise the product of all mutual pairwise
Euclidean distances
\begin{equation} \label{eq:product.mutual.distances}
\mathop{\prod_{i=1}^N \prod_{j=1}^N}_{i \neq j} \left\| \PT{x}_i-\PT{x}_j\right\|,
\end{equation}
or equivalently, minimise the discrete logarithmic energy 
\begin{equation*}
E_{\log}( \PT{x}_1, \dots, \PT{x}_N )\DEF
\mathop{\sum_{i=1}^N\sum_{j=1}^N}_{i \neq j} \log \frac{1}{\left\| 
\PT{x}_i - \PT{x}_j \right\|}
\end{equation*}
over all $N$-point configurations $( \PT{x}_1, \dots, \PT{x}_N )$ on
$\mathbb{S}^d$.
%
% In case of the $2$-sphere one can rewrite the
% product~\eqref{eq:product.mutual.distances} as
The discrete logarithmic energy is the limiting case (as $s \to 0$) of the
Riesz $s$-energy
\begin{equation*}
E_s( \PT{x}_1, \dots, \PT{x}_N ) \DEF 
\mathop{\sum_{i=1}^N\sum_{j=1}^N}_{i\neq j}
\frac{1}{\left\|\PT{x}_i-\PT{x}_j\right\|^s}.
\end{equation*}
The discrete Riesz $s$-energy problem for $s > 0$ is concerned with the
properties of $N$-point configurations $\{ \PT{x}_1^*, \dots, \PT{x}_N^* \}
\subset \mathbb{S}^d$ that minimise the Riesz $s$-energy over all $N$-point
configurations $( \PT{x}_1, \dots, \PT{x}_N )$ on $\mathbb{S}^d$. For
convenience we set $\kKERNEL_{s}( \PT{x}, \PT{y} ) \DEF - \log \| \PT{x} -
\PT{y} \|$ for $s = \log$ and $\kKERNEL_{s}( \PT{x}, \PT{y} ) \DEF 1 / \|
\PT{x} - \PT{y} \|^s$ for $s \in \R$. Then for $N \geq2$ we are interested in
the \emph{optimal $N$-point $s$-energy} of a compact set $A \subset \R^{d+1}$
defined by
\begin{equation*}
\mathcal{E}_s( A; N ) \DEF 
\begin{cases}
\min\big\{ E_s( \PT{x}_1, \dots, \PT{x}_N ) \, \mid \, 
\PT{x}_1, \dots, \PT{x}_N \in A \big\} & \text{for $s = \log$ or $s > 0$,} \\
\max\big\{ E_s( \PT{x}_1, \dots, \PT{x}_N ) \, \mid \, 
\PT{x}_1, \dots, \PT{x}_N \in A \big\} & \text{for $s < 0$.}
\end{cases}
\end{equation*}
% Observe that $\mathcal{E}_0( A; N ) = N^2 - N$ (which is attained by any
% $N$-point set on $A$).
The Riesz $s$-kernel is conditionally positive definite of order $1$ for $-2 <
s < 0$. Alternatively, as in the setting of numerical integration on
$\mathbb{S}^d$, one can  minimise
\begin{equation*}
2 \int_A \int_A \left\| \PT{x} - \PT{y} \right\|^{-s} 
\dd \sigma_d( \PT{x} \dd \sigma_d( \PT{y}) -
\mathop{\sum_{i=1}^N \sum_{j=1}^N} \left\| \PT{x}_i - \PT{x}_j \right\|^{-s}
\end{equation*}
in this case.

The \emph{$s$-potential} and the \emph{$s$-energy} of a measure $\mu$ in the
class $\mathcal{M}(A)$ of Borel probability measures supported on $A$ are
given, respectively, by
\begin{equation} \label{eq:potential.energy.integral}
U_s^{\mu}( \PT{x} ) \DEF \int_A \kKERNEL( \PT{x}, \PT{y} ) \, 
\dd \mu( \PT{y} ), \quad \PT{x} \in \R^{d+1}, \qquad \mathcal{I}_s( \mu ) 
\DEF \int_A \int_A \kKERNEL( \PT{x}, \PT{y} ) \, \dd \mu( \PT{x} ) 
\dd \mu( \PT{y} ).
\end{equation}
The \emph{$s$-capacity} of $A$ is for $s > 0$ the reciprocal of the Wiener
energy ${\inf\{ \mathcal{I}_s( \mu ) \mid \mu \in \mathcal{M}( A ) \}}$. (If
the Wiener energy is finite, it will be denoted by~$W_s(A)$.)
% Because of the possibility of negative logarithmic energy integral, we set
The logarithmic capacity is defined by
${\CAP_{\log}( A ) \DEF \exp( {-\inf\{ \mathcal{I}_{\log}( \mu ) \mid \mu \in
    \mathcal{M}( A ) \} })}$. The infimum is denoted by
$W_{\log}(A)$, if it is finite.
%
The lower semi-continuous logarithmic kernel is bounded from below and thus the
kernel $\kKERNEL_s$ (plus a constant if needed) is strictly positive definite
for $s = \log$ and $0 < s < p$. Consequently, the $s$-equilibrium measure
$\mu_{A,s}$ on $A$ is unique for every compact set $A \subset \R^p$ with finite
$s$-energy; cf.
\cite{Landkof1972:potential_theory,BoHaSaBook}. %(i.e. positive $s$-capacity).
For the range $-2 < s < 0$, one also has a unique $s$-equilibrium measure on
$A$; cf.~\cite{Bj1956} for the potential theoretic quantities and variational
inequalities.

An \emph{external field} will be a lower semi-continuous function
$\extFIELD:\mathbb{S}^d \to (-\infty,\infty]$ such that ${\extFIELD(\PT{x})<\infty}$ on a set
of positive Lebesgue surface measure. We note that the lower semi-continuity
implies the existence of a finite $c_\extFIELD$ such that $\extFIELD(\PT{x})\geq c_\extFIELD$ for all
$\PT{x}\in \mathbb{S}^d$. The {\em weighted energy associated with $\extFIELD(\PT{x})$}
is then given by
\begin{equation} \label{energy}
I_{\extFIELD,s}(\mu) \DEF \mathcal{I}_s(\mu) + 2 \int \extFIELD(\PT{x}) \dd \mu(\PT{x}), 
\qquad \mu \in \mathcal{M}( \mathbb{S}^d ).
\end{equation}
We recall from~\cite{Dragnev_Saff2007:riesz_potential_separation} the following
Frostman-type result which deals with existence and uniqueness of the
$s$-extremal measure on $A$ associated with $\extFIELD$ and its
characterisation in terms of weighted potentials.
%
The potential theory used in the context of this survey can be found in
G.~Bj{\"o}rck~\cite{Bj1956} (dealing with Riesz potential with negative
exponent), E.~B.~Saff and V.~Totik~\cite{Saff_Totik1997:logarithmic_potentials}
(logarithmic external field problem in the plane),
N.~S.~Landkof~\cite{Landkof1972:potential_theory} (Riesz and logarithmic
potential and general reference) and, in particular, for Riesz external field
problems N.~V.~Zori{\u\i}~\cite{Zo2003, Zo2004}.
%
\begin{prop} \label{prop:1} Let $0< s < d$.\footnote{A similar result holds for
    the logarithmic case.} For the minimal energy problem on $\mathbb{S}^d$
  with external field $\extFIELD$ the following properties hold:
\begin{itemize}
\item[\rm (a)] $W_{\extFIELD,s}$ is finite.
\item[\rm (b)] There exists a unique $s$-extremal measure $\mu_{\extFIELD,s}\in
  \mathcal{M}(\mathbb{S}^d)$ associated with $\extFIELD$.  Moreover, the support
  $S_{\extFIELD,s} \DEF \supp( \mu_{\extFIELD,s} )$ of this measure is contained in the compact
  set $E_M \DEF \{ \PT{x} \in \mathbb{S}^d : \extFIELD(\PT{x}) \leq M \}$ for some
  $M>0$.
\item[\rm (c)] The measure $\mu_{\extFIELD,s}$ satisfies the variational inequalities
\begin{align}
U_s^{\mu_{\extFIELD,s}}(\PT{x}) + \extFIELD(\PT{x}) &\geq F_{\extFIELD,s} \quad \text{q.e. on $\mathbb{S}^d$,} \label{VarEq1} \\
U_s^{\mu_{\extFIELD,s}}(\PT{x}) + \extFIELD(\PT{x}) &\leq F_{\extFIELD,s} \quad
\text{everywhere on $S_{\extFIELD,s}$,} \label{VarEq2}
\end{align}
where
\begin{equation}
F_{\extFIELD,s} \DEF W_{\extFIELD,s} - \int \extFIELD(\PT{x}) \dd \mu_{\extFIELD,s}(\PT{x}).
\label{VarConst}
\end{equation}
\item[\rm (d)] Inequalities \eqref{VarEq1} and
\eqref{VarEq2} completely characterise the $s$-extremal measure
$\mu_\extFIELD$ in the sense that if $\nu \in \mathcal{M}(\mathbb{S}^d)$ is
a measure with finite $s$-energy such that for some constant $C$ we
have
\begin{align}
U_s^{\nu}(\PT{x}) + \extFIELD(\PT{x}) &\geq C \quad \text{q.~e. on $\mathbb{S}^d$,} 
\label{VarEq3} \\
U_s^{\nu}(\PT{x}) + \extFIELD(\PT{x}) &\leq C \quad \text{everywhere on $\supp (\nu)$,}
\label{VarEq4}
\end{align}
then $\nu=\mu_{\extFIELD,s}$ and $C=F_{\extFIELD,s}$.
\end{itemize}
\end{prop}
We recall that a property is said to hold \emph{quasi everywhere} (``q.~e.'' for
short), if it holds outside of a set of zero capacity.

Observe that, if the external field $\extFIELD$ is continuous on $\mathbb{S}^d$, then
the inequality in \eqref{VarEq3} holds everywhere on $\mathbb{S}^d$.


\subsection{The distribution of minimal logarithmic and Riesz
energy points}
\label{sec:distribution.min.energy}

Let $A$ be an infinite compact set $A \subset \R^p$ with Hausdorff dimension
$d$ having finite logarithmic or Riesz $s$-energy and $\extFIELD \equiv
0$. Classical potential theory implies that the minimal energy $N$-point
configurations $X_N^*$ on~$A$ are distributed according to the unique
equilibrium measure $\mu_A$ on $A$ and the discrete measures $\mu_{X_N^*}$ will
have $\mu_A$ as a weak limit.
%
% the minimal energy $N$-point configuration will be distributed according the
% equilibrium measure $\mu_A$ on $A$ and tending to $\mu_A$ in the weak limit
% as $N \to \infty$.
%
Except for the unit sphere $\mathbb{S}^d$, this will be {\bf not} the
normalised uniform measure on $A$. This phenomenon can be observed particularly
well in the case of the circular torus $A = \mathbb{T}^2$. D.~P.~Hardin,
E.~B.~Saff and H.~Stahl~\cite{Hardin_Saff_Stahl2007:support_logarithmic} showed
that the logarithmic equilibrium measure $\mu_{\mathbb{T}}$ on the torus
$\mathbb{T}^2$ is supported on a proper subset of the surface part with
positive curvature. (The precise form of the logarithmic measure on the torus
is still unknown.)
%
Moreover, it could be shown
in~\cite{Brauchart_Hardin_Saff2007:riesz_energy_revolution,
  Brauchart_Hardin_Saff2009:riesz_energy_revolution} that the support of the
Riesz $s$-equilibrium measure on $\mathbb{T}$ for small $s > 0$ is a proper
subset of the torus. On the other hand, it is well-known
(cf.~Landkof~\cite{Landkof1972:potential_theory}) that in the harmonic case
($s=d-1$) the support of the equilibrium measure is always all of~$A$.
%
In general, the equilibrium measure $\mu_A$ will be supported on part of the
\emph{outer boundary} (i.e., the boundary of $A$ shared with the unbounded
component of the ambient space $\mathbb{R}^p$) if the energy kernel is strictly
superharmonic, all of the outer boundary if the kernel is harmonic and
supported on (part of) the volume as well if the kernel is strictly
subharmonic. Consequently, the minimal energy points are forced out of the
volume (if there is one) onto the outer boundary in the first case, spread out
over all of the outer boundary as their number increases (the ``interior''
becomes effectively field-free, ``Faraday-cage effect'') and in part injected
into the volume (if there is one) to decrease the discrete energy in the last
case.
%
This is the potential theoretic regime of D.~P.~Hardin and E.~B.~Saff's
\emph{Poppy-seed Bagel Theorem} where the poppy seeds represent the minimal
energy points and the Bagel is an interesting manifold.
%
The intuition is that in this regime $s = \log$ or $0 < s < d$ ($d$ the
Hausdorff dimension of~$A$) global effects dominate (points interact as if they
are subject to long-range forces and the range increases as $s$ becomes
smaller).
%
In the hypersingular case $s > d$, local effects dominate (points interact as
if they are responding to a short range force). Both kind of interaction
intermingle when $s = d$.

The energy integral diverges for every probability measure supported on
$\mathbb{S}^d$ in the hypersingular case $s \geq d$. Techniques from geometric
measure theory were applied to obtain that the limiting distribution of the
minimal Riesz $s$-energy $N$-point sets 
on $A$ (even asymptotically $s$-energy minimising would suffice) is uniformly
distributed with respect to the $d$-dimensional Hausdorff measure
$\mathcal{H}_d$; i.e.,
\begin{equation*}
  \mu_{X_N^*} \rightharpoonup \frac{\dd \mathcal{H}_d\big|_A}{\mathcal{H}_d(A)}
 \qquad N \to \infty, 
\end{equation*}
where $X_N^*$ are minimal $N$-point Riesz $s$-energy configurations on $A$ ($s
> \dim( A )$ and $\mathcal{H}_d( A ) > 0$) and, say, $A$ is a rectifiable set
(see~\cite{Borodachov_Hardin_Saff2008:asymptotics_riesz} and earlier
work~\cite{Borodachov_Hardin_Saff2007:asymptotics_best-packing,
Hardin_Saff2005:minimal_riesz,Hardin_Saff2004:discretizing_manifolds}). It
should be noted that in the case $s = \dim(A)$ an additional regularity
assumption on $A$ is required. The
paper~\cite{Borodachov_Hardin_Saff2008:asymptotics_riesz} also shows analogue
results for weighted Riesz $s$-energy
\begin{equation*}
\mathop{\sum_{i=1}^N \sum_{j=1}^N}_{i \neq j} 
\frac{w( \PT{x}_i, \PT{x}_j)}{\left\| \PT{x}_i - \PT{x}_j \right\|^s},
\end{equation*}
where $w$ is a CPD weight function (CPD stands for (almost everywhere)
continuous and positive on the diagonal).
%
We remark that the case $s = d$ for $\mathbb{S}^d$ has already been dealt with
in \cite{GoSa2001} using results in
\cite{Kuijlaars_Saff1998:asymptotics_minimal_energy}. Furthermore,
\cite{Calef_Hardin2009:riesz_equilibrium} showed that the $s$-equilibrium
measures on $A$ for $0 < s < d$ converge to the normalised $d$-dimensional
Hausdorff measure restricted to $A$ under rather general assumptions on $A$.
%
We remark that I.~Pritzker~\cite{Pr2011} studied the discrete approximation of
the equilibrium measure on a compact set $A \subset \R^p$, $p \geq 2$, with
positive $s$-capacity by means of points which do not need to lie inside
$A$. He also obtained discrepancy estimates in the harmonic case.


Summarising, for $-2 < s < 0$, $s = \log$ and $s > 0$, the (asymptotically)
$s$-energy minimising $N$-point configuration on $\mathbb{S}^d$ are uniformly
distributed with respect to the surface area measure $\sigma_d$.
%

In certain applications one would prefer to generate well-distributed $N$-point
sets on a compact $d$-rectifiable set in $\R^p$ which have a prescribed
non-uniform asymptotic distribution~$\rho$ with respect to $\mathcal{H}_d$ as
$N \to \infty$. It is shown in~\cite{HaSaWh2012} that such points can be
obtained by minimising the energy of $N$ points on $A$ interacting via a
weighted power law potential $w( \PT{x}, \PT{y} ) / \| \PT{x} - \PT{y} \|^s$,
where $s > d$ and $w( \PT{x}, \PT{y} ) \DEF [ \rho( \PT{x} ) \rho( \PT{y} )
]^{-s/(2d)}$; furthermore, such point sets are ``quasi-uniform'' in the sense
that the ratio of the covering radius (fill radius) to the separation distance
is uniformly bounded in $N$. As mentioned in the introduction, quasi-uniformity
is crucial for a number of numerical methods
(cf.~\cite{FuWr2009,LeGSlWe2010,Sch1995}).
% The covering radius appears in error estimates of numerical methods and
% separation is generally associated with the ``stability''. Thus
% quasi-uniformity is a crucial requirement for a number of methods. We refer
% the reader to~\cite{FuWr2009,LeGSlWe2010,Sch1995}.
S.~V.~Borodachov, D.~P.~Hardin and E.~B.~Saff show in
\cite{BoHaSa_arXiv:1305.6337v1} that it suffices to use a varying truncated
weight $w( \PT{x}, \PT{y}) \, \Phi( \| \PT{x} - \PT{y} \| / r_N )$, thus
keeping  only those pairs of points in the energy sums that are located at a
distance of at most $r_N = C_N \, N^{-1/d}$ from each other. (The positive
sequence $(C_N)$ tends to $\infty$ as slowly as desired.) In this way, under
suitable assumptions, the complexity of the energy computation can be greatly
reduced leading to order $N \, C_N^d$ computations for generating ``low
energy'' $N$-point approximations.

A point charge approaching the sphere subject to the same law of interaction as
the points on the sphere affects the charge distribution on the sphere. If the
point charge is sufficiently close to the sphere, it will free up a part of
charges. The papers \cite{BrDrSa2009,BrDrSa2012,BrDrSa2014}, in particular,
provide explicit representations of the charge distributions due to a canonical
single external charge. They also address a question attributed to
A.~A.~Gonchar, namely to find a critical distance of the external field
generating charge from the sphere surface so that the support of the
$s$-extremal measure on $\mathbb{S}^d$ for this external field is just all of
the sphere. In the harmonic case this distance is characterised by a zero of a
class of polynomials dubbed Gonchar polynomials. (The golden ratio and the
plastic number play a prominent role for $d = 2$ and $d =4$.)

% For small number of points numerical 


\subsection{Asymptotic expansion of minimal Riesz energy}
\label{sec:asympt-expans-minim}
%
Let $s > 0$. 
%
The leading term of the asymptotic expansion for a compact set $A$ in $\R^p$ is
well-understood if $A$ has positive $s$-capacity (i.e., finite Riesz
$s$-energy). This is the \emph{potential-theoretic regime}. A standard argument
from classical potential theory yields that the positive quantities ${N ( N - 1
  ) / \mathcal{E}_s( A; N )}$ form a monotonically decreasing sequence. The
limit $\TFDIAM_s( A )$, called the \emph{generalised transfinite diameter of
  $A$}, is equal to the $s$-capacity of $A$
(cf.~\cite{Polya_Szego:transfiniten_durchmesser}). Thus, the leading term of
$\mathcal{E}_s( A; N )$ grows like $N^2$ as $N \to \infty$ and the leading
coefficient is given by the Riesz $s$-energy of $A$, or equivalently, by the
reciprocals of the $s$-capacity and transfinite diameter of $A$:
% encodes the Riesz $s$-energy, the $s$-capacity and the transfinite diameter
% of $A$ by means of
\begin{equation}
\lim_{N \to \infty} \frac{\mathcal{E}_s( A; N )}{N^2} = W_s( A ) =
\frac{1}{\CAP_s( A )} = \frac{1}{\TFDIAM_s( A )}. 
%,  \qquad \text{$-2 < s < 0$ or $0 < s < d$.} 
\end{equation}
For $0 < s < d$, the Riesz $s$-energy of the sphere $\mathbb{S}^d$ has the
explicit form
\begin{equation} \label{eq:W.s.sphere}
W_s( \mathbb{S}^d ) = \mathcal{I}_s[ \sigma_d ] = 
2^{d-1-s} \frac{\gammafcn( ( d + 1 ) / 2 ) \, 
\gammafcn( ( d - s ) / 2 )}{\sqrt{\pi} \, \gammafcn( d - s / 2 )},
\end{equation}
expressed in terms of the Gamma function $\gammafcn$. By identifying $W_s(
\mathbb{S}^d )$ with the analytic continuation of the right-hand side above to
the complex $s$-plane\footnote{The meromorphic function $W_s( \mathbb{S}^d )$,
  which appears in the conjecture for the asymptotics in the hypersingular
  case, has simple poles (finitely many if $d$ is even and infinitely many if
  $d$ is odd). The effect of this dichotomy on the asymptotic expansion of the
  minimal Riesz $s$-energy is completely open for $d \geq 2$ and leads to $\log
  N$ terms for the unit circle,
  cf.~\cite{Brauchart_Hardin_Saff2009:riesz_energy_roots}.}, we can define the
Riesz $s$-energy of $\mathbb{S}^d$ for Riesz parameter $s$ for which the
$s$-energy integral \eqref{eq:potential.energy.integral} is~$+\infty$ for every
Borel probability measure on $\mathbb{S}^d$.
%
% of this meromorphic function in the complex $s$-plane. We shall use the
% symbol $W_s( \mathbb{S}^d )$ for this extension.
%
% The $s$-energy integral \eqref{eq:energy.integral} is~$+\infty$ for every
% Borel probability measure on $\mathbb{S}^d$ if $s > d$.
% 
% (Note that the $s$-energy integral \eqref{eq:energy.integral} is~$+\infty$
% for every Borel probability measure on $\mathbb{S}^d$ if $s > d$, however,
% the right-hand side above is a meromorphic function in the complex $s$-plane
% with simple poles\footnote{There are finitely many poles if $d$ is even and
% infinitely many if $d$ is odd.}. We shall use the same symbol $W_s(
% \mathbb{S}^d )$ for this extension.)
%
% The large $N$ behavior of the minimal Riesz $s$-energy $\mathcal{E}_s(
% \mathbb{S}^d, N )$ is qualitatively different for the potential theoretic
% regime $0 < s < d$ (and $-2 < s < 0$) and for the hypersingular cases $s = d$
% and $s > d$. Classical potential theory yields that for $-2 < s < 0$ or $0 <
% s < d$,
% \begin{equation*}
% \lim_{N \to \infty} \frac{\mathcal{E}( \mathbb{S}^d; N )}{N^2} = 
% W_s( \mathbb{S}^d ). %,  \qquad \text{$-2 < s < 0$ or $0 < s < d$.} 
% \end{equation*}
%
The combined effort of \cite{Wagner1992:means_distances_upper,
  Rakhmanov_Saff_Zhou1994:minimal_discrete_energy,
  Kuijlaars_Saff1998:asymptotics_minimal_energy,
  Wagner1990:means_distances_lower, Brauchart2006:riesz_energy} resulted in the
following bounds for the second term of the minimal energy
asymptotics\footnote{Similar estimates but with negative constants $c, C$
  holds for the sum of generalised distances (i.e.,~${-2 < s < 0}$);
  cf.~\cite{Al1972, Al1977, Stolarsky1973:sums_distances_ii, Ha1982, Be1984,
    Stolarsky1972:sums_distances_i, AlSt1974} and culminating
  in~\cite{Wagner1990:means_distances_lower,
    Wagner1992:means_distances_upper}.}: There exist constants $c, C > 0$
depending only on $d \geq 2$ and $0 < s < d$ such that
\begin{equation*}
c \, N^{1+s/d} \leq \mathcal{E}_s( \mathbb{S}^d; N ) - 
W_s( \mathbb{S}^d ) \, N^2 \leq C \, N^{1+s/d}, \qquad N \geq 2.
\end{equation*}
This estimates give the correct order of growth and sign for the second-order
term. It is an open problem if the sequence $\big( \mathcal{E}_s( \mathbb{S}^d;
N ) - W_s( \mathbb{S}^d ) \, N^2 \big) / N^{1+s/d}$ has a limit as $N \to
\infty$. A.~A.~Berezin~\cite{Be1986} used a semicontinuum approach (a classical
method from solid state physics, cf.~\cite{GoAd1960}) to derive the plausible
asymptotics
\begin{equation*}
\begin{split}
\mathcal{E}_s( \mathbb{S}^2; N ) 
&\approx N^2 \frac{2^{1-s}}{2-s} \left[1 -\left( n / N \right)^{1-s/2} \right] 
+ N^{1+s/2} \left( \frac{\sqrt{3}}{8 \pi} \right)^{s/2} \\
&\phantom{=\pm\times}\times \left\{ \frac{6}{1^s} + \frac{6}{( \sqrt{3} )^s} 
+ \frac{6}{2^s} + \frac{12}{( \sqrt{7} )^s} + \frac{6}{3^s} + 
\frac{6}{( 2 \sqrt{3} )^s} + \frac{12}{( \sqrt{13} )^s} + \cdots \right\}
\end{split}
\end{equation*}
based on the assumptions that a typical point (and most of its immediate
neighbours) in a minimal Riesz $s$-energy $N$-point configuration on
$\mathbb{S}^2$ gives rise to a hexagonal Voronoi cell (sixfold symmetry)
whereas the defects according to the curved surface of the sphere will have no
significant role for the second term in the asymptotics. Thus the contribution
to the Riesz $s$-energy due to a typical point can be split into a local part
which uses $n$ nearest neighbour points from a suitably adjusted (thus the
geometric scaling factor) flat hexagonal lattice and a distant part where the
$N-n$ points are replaced by the continuous uniform distribution. The
expression in curly braces gives the formal series expansion of the Epstein
zeta function of the hexagonal lattices truncated to include only the $n-1$
shortest distances in the lattice\footnote{Indeed, the first few most frequent
  distances in a putative minimal energy configuration emulate remarkably well
  the first few distances in a hexagonal lattice (cf., in particular,
  \cite[Figure~1]{ Brauchart_Hardin_Saff2012:riesz}).}.
%
(In order to get a non-trivial expansion, $n$ has to grow weakly to
infinity. The paper~\cite{Be1986} mentions some numerical experiments for
slowly growing $n$ but a rigorous investigation has not been undertaken.) The
discussion leading to Conjecture~\ref{conj:d.2.4.8.24} below suggests that
the semicontinuum approach would also work for $d = 4$, $8$ and $24$. In
general, it is not clear what local approximation should be used.

For a compact set $A$ in $\R^p$ of vanishing $s$-capacity, the leading term is
rather well-understood. In the \emph{(strictly) hypersingular regime $s > d$},
where $d$ is the Hausdorff dimension of $A$, Hardin and
Saff~\cite{Hardin_Saff2005:minimal_riesz} (for rectifiable $d$-dimensional
manifolds including the sphere $\mathbb{S}^d$) and Borodachov, Hardin and
Saff~\cite{Borodachov_Hardin_Saff2008:asymptotics_riesz} (for infinite compact
$d$-rectifiable sets\footnote{A $d$-rectifiable set is the Lipschitz image of a
  bounded set in $\R^d$.}) established for a large class of compact sets $A$
the existence of a constant $C_{s,d}$ such that\footnote{The boundedness of
  $\mathcal{E}_s( \mathbb{S}^d; N ) / N^{1+s/d}$ has already been shown
  in~\cite{Kuijlaars_Saff1998:asymptotics_minimal_energy}.}
%
\begin{equation} \label{eq:Poppy.seed.Bagel.Theorem}
\lim_{N \to \infty} \frac{\mathcal{E}_s( A; N )}{N^{1+s/d}} = 
\frac{C_{s,d}}{\left[ \mathcal{H}_d( A ) \right]^{s/d}}.
\end{equation}
This result is also referred to as the \emph{Poppy-seed Bagel Theorem} because
of its interpretation for distributing points on a
torus.\footnote{Cf.~\url{http://news.vanderbilt.edu/2004/11/the-poppy-seed-bagel-theorem-59497/}}
%
Here and hereafter, $\mathcal{H}_d$ denotes the $d$-dimensional Hausdorff
measure in $\R^p$ normalised such that the $d$-dimensional unit cube has
$\mathcal{H}_d$-measure $1$. Except for one-dimensional sets (when $C_{s,1}$ is
twice the Riemann zeta function at $s$, see~\cite[Thm.~3.1]{MaMaRaSa2004}), the
precise value of $C_{s,d}$ is not known. Its determination is a challenging
open problem. The significance and difficulty of obtaining $C_{s,d}$ is due to
the deep connection to densest
packings. In~\cite{Borodachov_Hardin_Saff2007:asymptotics_best-packing} it is
shown that $C_{s,d}$ is tied to the largest sphere packing density $\Delta_d$
in~$\R^d$ and the best-packing distance $\delta_N^*$ of $N$-points on
$\mathbb{S}^d$ by means of the limit relations\footnote{Indeed, one can recasts
  this relation as $\Delta_d = \lim_{s \to \infty} \lim_{N \to \infty} \big[
  \mathcal{E}_s( \frac{1}{2} \mathbb{B}^d; N ) / N^{1+s/d} \big]^{-d/s}$.}
%
\begin{equation} \label{eq:density.limit.relations}
\lim_{s \to \infty} \left[ C_{s,d} \right]^{-1/s} = 
2 \left[ \frac{\Delta_d}{\mathcal{H}_d( \mathbb{B}^d )} \right]^{1/d} 
= \lim_{N \to \infty} N^{1/d} \delta_N^*.
\end{equation}
%
(Here, $\mathcal{H}_d( \mathbb{B}^d )$ is the volume of the unit ball in
$\R^d$.) We recall that $\Delta_d$ is only known for three cases: $\Delta_1=1$,
$\Delta_2 = \pi / \sqrt{12}$ (A.~Thue in 1892 and L.~Fejes
T{\'o}th~\cite{Fe1972}) and $\Delta_3=\pi/\sqrt{18}$ (Kepler conjecture proved
by Hales~\cite{Hales2005:kepler_conjecture}). The connection to (regular)
lattices is evident in the upper estimate of the constant $C_{s,d}$ in terms of
the Epstein zeta function $\zetafcn_\Lambda( s )$ of a lattice $\Lambda$ in
$\mathbb{R}^d$ which can be obtained by considering the Riesz $s$-energy of the
$N = n^d$ points of the rescaled lattice $\frac{1}{n} \Lambda$ lying in the
fundamental parallelotope $\Omega$ of $\Lambda$ and which implies that
$\mathcal{E}_s( \Omega; N ) \leq n^{d+s} \zetafcn_\Lambda( s ) = N^{1 + s / d}
\zetafcn_\Lambda( s )$ and thus for $s > d$
(cf.~\cite[Prop.~1]{Brauchart_Hardin_Saff2009:riesz_energy_roots}),
%
\begin{equation} \label{eq:C.s.d..Epstein.zeta.fcn}
C_{s,d} \leq \min_\Lambda \left| \Lambda \right|^{s/d} \zetafcn_\Lambda( s ),
\end{equation}
%
where the minimum is extended over all lattices $\Lambda$ in $\R^d$ with
positive covolume $| \Lambda |$.
%
Because of \eqref{eq:density.limit.relations}, the sharpness of this inequality
touches on questions regarding densest lattice sphere packings and which (if
so) solve the sphere packing problem.
%
For ${1 \leq d \leq 8}$ and $d = 24$, the unique densest lattice in $\R^d$ up
to scaling and isometries is the root lattice $A_1$, $A_2$, $A_3$, $D_4$,
$D_5$, $E_6$, $E_7$, $E_8$ and the Leech lattice, respectively
(cf.~\cite{Cohn_Kumar2009:optimality_leech}). Among those the hexagonal lattice
$A_2$ in $\R^2$, the $E_8$ root lattice in $\R^8$ and the Leech lattice
in~$\R^{24}$ are conjectured to be optimal for all values of $s>d$
(\emph{universally optimal}) whereas the remaining lattices are provably not
universally optimal (cf.~\cite{Cohn_Kumar2007:universally_optimal_sphere,
  CohnKumarSchurmann}). See \cite{Sarnak_Stroembergsson2006:minima_epsteins}
for local optimality results and
\cite{Coulangeon_Schuermann2012:energy_minimization} for improvements.
%
Montgomery~\cite{Montgomery1988:minimal_theta} proved that the hexagonal
lattice is universally optimal among all lattices in $\R^2$ (which is weaker
than universal optimality among all periodic point configurations). Cohn and
Elkis~\cite{Cohn_Elkies2003:bounds_sphere_packings_i} conjectured that $E_8$
and the Leech lattice solve the sphere packing problem in their dimension.
%
It is generally expected that for sufficiently large $d$, lattice packings are
not densest packings and \cite{ToSt2006} suggests that best-packings are highly
``disordered'' as $d \to \infty$. This motivates the following
conjecture\footnote{The conjecture for $d = 2$ appeared
  in~\cite{Kuijlaars_Saff1998:asymptotics_minimal_energy}.}.
%
% Indeed, from \cite{ToSt2006} one would expect that best-packings are highly
% ``disordered'' and thus equality would not hold in
% \eqref{eq:C.s.d..Epstein.zeta.fcn} for most $d$. On the other hand, the
% results and conjectures
% in~\cite{Cohn_Elkies2003:bounds_sphere_packings_i,
% Cohn_Kumar2007:universally_optimal_sphere,CohnKumarSchurmann}
% (cf. also~\cite{Montgomery1988:minimal_theta,
% Sarnak_Stroembergsson2006:minima_epsteins})
% suggest the following\footnote{The conjecture for $d = 2$ appeared
% in~\cite{Kuijlaars_Saff1998:asymptotics_minimal_energy}.}.
%
\begin{conjecture}[\cite{Brauchart_Hardin_Saff2009:riesz_energy_roots}] 
\label{conj:d.2.4.8.24}
  For $d = 2$, $4$, $8$ and $24$, one has $C_{s,d} = \left| \Lambda_d
  \right|^{s/d} \zetafcn_{\Lambda_d}( s )$, where $\Lambda_d$ denotes,
  respectively, the hexagonal lattice $A_2$, the root lattices $D_4$ and $E_8$,
  and the Leech lattice.
\end{conjecture}

We remark that in \cite{Brauchart_Hardin_Saff2012:riesz} very coarse lower and
upper bounds are obtained for $\mathcal{E}_s( \mathbb{S}^d; N )$. Although, the
leading term has the wrong coefficient, curiously, the second order term in the
lower bound has the conjectured form. As a consequence of these bounds,
\cite{Brauchart_Hardin_Saff2012:riesz} could give the  estimates
\begin{equation*}
  \frac{d}{s-d} \left[ \frac{1}{2} 
\frac{\gammafcn((d+1)/2) \gammafcn(1+(s-d)/2)}{\sqrt{\pi}\gammafcn(1+s/2)} 
\right]^{s/d} \leq 
\frac{C_{s,d} }{ \left[ \mathcal{H}_d(\mathbb{S}^d) \right]^{s/d}} \leq 
\left[ 
\frac{\mathcal{H}_d(\mathbb{B}^d)}{\mathcal{H}_d(\mathbb{S}^d)( 1-d/s )}
\right]^{s/d},
\end{equation*}
valid for $s > d \geq 2$ and $(s-d)/2$ not an integer.

In the \emph{hypersingular case $s = d$}, where $d$ is the Hausdorff dimension
of the compact set~$A$ in $\R^p$, much more can be said. For a wide family of
compact sets $A$, this boundary case can still be treated using a suitably
renormalised energy integral and a limit process as $s$ approach $d$ from below
(i.e., from the potential theoretic regime),
cf.~\cite{Calef_Hardin2009:riesz_equilibrium}. It has been known
since~\cite{Kuijlaars_Saff1998:asymptotics_minimal_energy} that the leading
term of $\mathcal{E}_d( \mathbb{S}^d; N )$ grows like $N^2 \log N$ and
\begin{equation}
\lim_{N \to \infty} \frac{\mathcal{E}_d( \mathbb{S}^d; N)}{N^2 \log N} = 
\frac{\mathcal{H}_d(\mathbb{B}^d)}{\mathcal{H}_d(\mathbb{S}^d)} = 
\frac{1}{d} \frac{\omega_{d-1}}{\omega_{d}} = 
\frac{1}{d} \frac{\gammafcn((d+1)/2)}{\sqrt{\pi} \gammafcn(d/2)}.
\end{equation}
The best estimates so far for the second-order term has been obtained recently
in~\cite{Brauchart_Hardin_Saff2012:riesz},
%
% Let $d \geq 2$. Then, as $N \to \infty$,
\begin{equation*} 
- c(d) \, N^2 + \mathcal{O}(N^{2-2/d} \log N)\le 
\mathcal{E}_d( \mathbb{S}^d; N )-
\frac{\mathcal{H}_d(\mathbb{B}^d)}{\mathcal{H}_d(\mathbb{S}^d)} \, N^2 \log N  
\leq   \frac{\mathcal{H}_d(\mathbb{B}^d)}{\mathcal{H}_d(\mathbb{S}^d)} \, N^2 
\log \log N + \mathcal{O}(N^2)  
\end{equation*}
as $N \to \infty$, where the constant $c(d)$ is given by 
\begin{equation*}
  c(2) = 1/2, \qquad c(d) \DEF 
\frac{\mathcal{H}_d(\mathbb{B}^d)}{\mathcal{H}_d(\mathbb{S}^d)} 
\left\{ 1 - \log \frac{\mathcal{H}_d(\mathbb{B}^d)}
{\mathcal{H}_d(\mathbb{S}^d)} + d \left[ \digammafcn(d/2) - 
\digammafcn(1) - \log 2 \right] \right\} > 0.
\end{equation*}
(Recall, that $\digammafcn=\gammafcn'/\gammafcn$ denotes the digamma function.)
The paper~\cite{Brauchart_Hardin_Saff2012:riesz} conjectures, based on a limit
process $s \to d$ in Conjecture~\ref{conj:fundamental.conj}, that the correct
order of the second term is $N^2$ and provides a limit relation for the
constant which is made explicit for the case $d = 2$.


\subsubsection*{Higher Order Terms -- Complete Asymptotic 
Expansions --  Fundamental Conjecture}


Almost nothing is known about higher-order terms of the asymptotics of the
minimal Riesz $s$-energy except for the unit circle. As the $N$-th roots of
unity are universally optimal\footnote{For $s \geq -1$ (and $s \neq 0$) a
  convexity argument can be applied to get optimality for Riesz $s$-energy
  (cf.~\cite{AlSt1974,Fe1964,Go2003}). The much more general
  result~\cite[Theorem~1.2]{Cohn_Kumar2007:universally_optimal_sphere} provides
  optimality for $s > -2$.},
%
the complete asymptotic expansion can be obtained by direct computation of the
Riesz $s$-energy $\mathcal{L}_s( N )$ of the $N$-th roots of unity,
see~\cite{Brauchart_Hardin_Saff2007:riesz_energy_revolution} (and
cf.~\cite{BrHaSa2012} for geodesic distance). Indeed, for $s \in \C$ with $s
\neq 0, 1, 3, 5, \dots$ and fixed $p = 1, 2, 3, \dots$, one has\footnote{The
  precise formulas for finite $N \geq 2$ are obtained in~\cite{Br2011arXiv}.}
\begin{equation} \label{eq:circle.asympt}
\begin{split}
\mathcal{L}_s(N) 
&= W_s(\mathbb{S}^1) \, N^2 + \frac{2\zetafcn(s)}{(2\pi)^s} \, N^{1+s} + 
\sum_{n=1}^p \alpha_n(s) \frac{2\zetafcn(s-2n)}{(2\pi)^s} \, N^{1+s-2n} \\
&\phantom{=\pm}+ \BigOh_{s,p}(N^{-1+\Re s-2p}) \qquad \text{as $N \to \infty$,}
\end{split}
\end{equation}
% where $\zetafcn(s)$ is the classical Riemann zeta function. 
where the coefficients $\alpha_n(s)$, $n\geq0$, satisfy the generating function
relation
\begin{equation*} \label{sinc.power.0}
\left( \frac{\sin \pi z}{\pi z} \right)^{-s} = 
\sum_{n=0}^\infty \alpha_n(s) \, z^{2n}, \quad |z|<1, \ s\in \C.
\end{equation*}
(Explicit formulas in terms of generalised Bernoulli polynomials
$B_n^{(\alpha)}(x)$ are given in~\cite{BrHaSa2012}.)
%
This expansion has two noteworthy features: 
\begin{inparaenum}[\upshape(\itshape i\upshape)]
\item the fact that the expansion is valid for complex $s$ and
\item the essential role played by the Riemann zeta function.
\end{inparaenum}
The former gives a unifying picture of the coefficients of the asymptotic
terms. They are best understood as functions in the complex $s$-plane
(\emph{principle of analytic continuation})\footnote{This principle breaks down
  when the perfectly symmetric unit circle is replaced by some other smooth
  closed curve $\Gamma$. Then the $s$-equilibrium measure on $\Gamma$ is not
  the normalised arc-length measure for each $0 < s < 1$ which plays a role in
  the characterisation of the coefficient of $N^2$ in the hypersingular regime
  $1 < s < 3$; cf.~\cite{Borodachov2012:lower_riesz}.}. The latter explains how
a logarithmic term arises as $s$ tends to one of the exceptional cases $1, 3,
5, \dots$, when the argument of one of the Riemann zeta functions approaches
the simple pole at $1$ and the associated term needs to be matched with the
$N^2$-term to offset the simple pole of $W_s( \mathbb{S}^1 )$.

By combining the results for the potential theoretic and the hypersingular
regime, the principle of analytic continuation motivates the following
fundamental conjecture.

\begin{conjecture}[{cf.~\cite{Brauchart_Hardin_Saff2012:riesz}}] 
\label{conj:fundamental.conj}
Let $d \geq 2$. Then for $0 < s < d + 2$ with $s \neq d$, 
%there exists a constant $C_d( s )$ such that
\begin{equation*}
\mathcal{E}_s( \mathbb{S}^d; N ) = W_s( \mathbb{S}^d ) \, N^2 + 
\frac{C_d( s )}{\left[ \mathcal{H}_d( A ) \right]^{s/d}} \, N^{1+s/d} + 
o( N^{1 + s/d} ) \qquad \text{as $N \to \infty$,}
\end{equation*}
where $W_s( \mathbb{S}^d )$ is the analytic continuation of the right-hand side
of~\eqref{eq:W.s.sphere} and $C_d( s )$ is the analytic continuation of
$C_{s,d}$ in \eqref{eq:Poppy.seed.Bagel.Theorem}. Furthermore, for $d = 2, 4,
8$ and $24$, $C_d( s )$ is the analytic continuation of $\left| \Lambda_d
\right|^{s/d} \zetafcn_{\Lambda_d}( s )$, where $\Lambda_d$ is given in
Conjecture~\ref{conj:d.2.4.8.24}.
\end{conjecture}
%  C_{s,d}



\subsection{Asymptotic expansion of logarithmic energy}
\label{sec:asympt-expans-minim.log}

The leading term of the asymptotic expansion for a compact set $A$ in $\R^p$
with positive logarithmic capacity (i.e. finite logarithmic energy) follows
from classical potential
theory. %A similar argument as in the Riesz case gives that the quantities
%
It should be noted that (cf.~\cite{BoHaSaBook})
\begin{equation} \label{eq:log.energy.diff}
\frac{\dd}{\dd s} \mathcal{E}_s( A; N ) \Big|_{s = 0^+} = 
\mathcal{E}_{\log}( A; N ),  \qquad N \geq 2.
\end{equation}
For the unit sphere $\mathbb{S}^d$ one has in particular that
\begin{equation*}
\lim_{N \to \infty} \frac{\mathcal{E}_{\log}( \mathbb{S}^d; N )}{N^2} = 
W_{\log}( \mathbb{S}^d ) = \log \frac{1}{\CAP_{\log}( \mathbb{S}^d )},
\end{equation*}
where the \emph{logarithmic energy of $\mathbb{S}^d$} is given by
\begin{equation*}
W_{\log}( \mathbb{S}^d ) = \frac{\dd W_s( \mathbb{S}^d )}{\dd s} \Big|_{s =0^+}
 = \log \frac{1}{2}+\frac{1}{2}\left[\digammafcn(d)-\digammafcn(d/2)\right].
\end{equation*}
Here, $\digammafcn$ is the digamma function. From an averaging argument
using equal-area partitions of $\mathbb{S}^d$ (cf.~\cite{Le2006}) and bounds of
G.~Wagner~\cite{Wagner1992:means_distances_upper} and the first
author~\cite{Brauchart2008:optimal_logarithmic} it follows that
\begin{equation*}
\mathcal{E}_{\log}( \mathbb{S}^d; N ) = W_{\log}( \mathbb{S}^d ) \, N^2 - 
\frac{1}{d} \, N \log N + \BigOh( N ), \qquad N \to \infty.
\end{equation*}
Relation~\eqref{eq:log.energy.diff} and Conjecture~\ref{conj:fundamental.conj}
provide the basis for the following conjecture proposed
in~\cite{Brauchart_Hardin_Saff2012:riesz}.

\begin{conjecture}
For $d = 2$, $4$, $8$ and $24$, 
\begin{equation*}
\mathcal{E}_{\log}( \mathbb{S}^d; N ) = W_{\log}( \mathbb{S}^d ) \, N^2 - 
\frac{1}{d} \, N \log N + C_{\log,d} \, N + o(N) \qquad 
\text{as $N \to \infty$,}
\end{equation*}
where 
\begin{equation*}
C_{\log,d} = \frac{1}{d} \log \frac{\mathcal{H}_d( \mathbb{S}^d )}{|\Lambda_d|} 
+ \zetafcn_{\Lambda_d}^\prime( 0 ).
\end{equation*}
For $d = 2$ one has
\begin{equation*}
C_{\mathrm{log},2} = 2 \log 2 + \frac{1}{2} \log \frac{2}{3} + 
3 \log \frac{\sqrt{\pi}}{\gammafcn(1/3)} = -0.05560530494339251850\dots < 0.
\end{equation*}
\end{conjecture}

For more details, we refer to~\cite{Brauchart_Hardin_Saff2012:riesz}.

% For the unit sphere 
% \begin{equation*}
% 
% \end{equation*}





\subsection{Numerical integration from the energy point of 
view}\label{sec:numer-integr-from}

The reproducing kernel Hilbert space approach (cf. Section~\ref{sec:designs})
allows to write the squared worst-case error as
\begin{equation*}
\sum_{i=1}^N \sum_{j=1}^N \KERNEL( \PT{x}_i, \PT{x}_j ) - 
\int_{\mathbb{S}^d} \int_{\mathbb{S}^d} \KERNEL( \PT{x}, \PT{y} ) \, 
\dd \sigma_d( \PT{x} ) \dd \sigma_d( \PT{y} )
\end{equation*}
which can be interpreted as $\KERNEL$-energy of the node set $\{ \PT{x}_1,
\dots, \PT{x}_N \}$ of the QMC method. The energy kernel here is a reproducing
kernel for $H^s( \mathbb{S}^d )$. Optimal nodes then can be obtained by solving
a minimal energy problem for this kernel. In
\cite{Brauchart_Dick2013:characterization_sobolev_spaces} and
\cite{Brauchart_Dick2013:stolarskys_invariance} it is shown how the distance
kernel
\begin{equation} \label{eq:K.gd.s}
\KERNEL_{\mathrm{gd}}^{(s)}( \PT{x}, \PT{y} ) \DEF 2 W_{d-2s}( \mathbb{S}^d ) - 
\left\| \PT{x} - \PT{y} \right\|^{2s-d},\qquad \PT{x},\PT{y}\in\mathbb{S}^d,
\end{equation}
arises in a natural way as a reproducing kernel for $H^s( \mathbb{S}^d )$ for
$s$ in $(d/2, d/2+1)$.
% when starting with the integral 
% \begin{equation*}
% \int_{-1}^1 \int_{\mathbb{S}^d} 
%\left( \PT{x} \cdot \PT{z} - t \right)_+^{\beta - 1} \left( \PT{y} \cdot 
% \PT{z} - t \right)_+^{\beta - 1} \dd \sigma_d( \PT{z} ) \dd t
% \end{equation*}
Wagner's bounds on the sum of generalised distances
(\cite{Wagner1990:means_distances_lower,Wagner1992:means_distances_upper})
yield that a sequence of $N$-point maximises of the generalised sum of
distances with power $2s-d$ and $N \to \infty$ form a QMC design sequence for
$H^s( \mathbb{S}^d )$, $d/2 < s < d/2 + 1$;
cf.~\cite{Brauchart_Saff_Sloan+2014:qmc-designs}.
%
For $s \geq d/2 + 1$, an equivalent norm on $H^s(\mathbb{S}^d)$ can be chosen
so that the corresponding reproducing kernel is essentially a distance kernel
with power $2s-d$. However, the kernel function $r^\alpha$ (for $\alpha>0$) is
only conditionally positive definite, whereas a reproducing kernel is always
positive definite (in the sense of
Schoenberg~\cite{Schoenberg1938:positive_definite}). This fact is taken care of
by introducing a logarithmic factor, if $s-d/2$ is a positive integer, and a
polynomial correction in general. In
\cite{Brauchart_Saff_Sloan+2014:qmc-designs} the correction term simply flips
the negative signs whereas
in~\cite{Brauchart_Dick2013:characterization_sobolev_spaces} the correction
term is induced by the considered integral representation of the reproducing
kernel.
%
% This particular issue with conditional positivity does not occur 
Such a correction term gets annihilated when the search for optimal QMC designs
for $H^s( \mathbb{S}^d )$, $s \in (d/2 + L, d/2 + 1 + L)$, $L$ a positive
integer, is restricted to spherical $L$-designs. In that case it suffices to
minimise the energy functional
(cf.~\cite{Brauchart_Saff_Sloan+2014:qmc-designs})
\begin{equation*}
\left[ \WCE_{H^s}(X_{N,L}) \right]^2 = 
\frac{1}{N^2} \sum_{i=1}^{N} \sum_{j=1}^{N} (-1)^{L+1} 
\left\| \PT{x}_{i,L} - \PT{x}_{j,L} \right\|^{2s-d} - 
(-1)^{L+1} W_{d-2s}(\mathbb{S}^d)
\end{equation*}
subject to the condition that the node set $X_{N,L} = \{ \PT{x}_{1,L}, \dots,
\PT{x}_{N,L} \} \subset \mathbb{S}^d$ is a spherical $L$-design. Note that $L$
depends on $s$ and is fixed, once $s$ is fixed. The value $L$ is ``small'' in
the following sense: a QMC method with a more regular (in the sense of
spherical designs) node set is more suitable for integrating functions from a
smoother function space $H^s(\mathbb{S}^d)$. But regularity beyond a critical
order will not improve the worst-case error bound; cf. optimal
order~\eqref{eq:wce2}.
%
We remark that the Cui and Freeden kernel
\cite{Cui_Freeden1997:equidistribution_sphere}
% \begin{equation*}
% \KERNEL_{\mathrm{CF}}(\PT{x}, \PT{y}) \DEF 2 - 2 \log\Big( 1 + \sqrt{ \frac{1-\PT{x}\cdot\PT{y}}{2}} \Big),\qquad \PT{x},\PT{y}\in\mathbb{S}^2,
% \end{equation*}
\begin{equation*}
\KERNEL_{\mathrm{CF}}(\PT{x}, \PT{y}) \DEF 
2 - 2 \log\Big( 1 + \frac{1}{2} \left\| \PT{x} - \PT{y} \right\| \Big),
\qquad \PT{x},\PT{y}\in\mathbb{S}^2,
\end{equation*}
can be interpreted as reproducing kernel for $H^{3/2}( \mathbb{S}^2 )$ as
observed in \cite{Sloan_Womersley2004:extremal_sphere} and the minimising
$\KERNEL_{\mathrm{CF}}$-energy point configurations give rise to a QMC design
sequence for $H^{3/2}( \mathbb{S}^2 )$. Recently, Choirat and
Seri~\cite{ChSe2013,ChSe2013b} derived the analogue kernel for $d$-spheres. The
corresponding minimising configurations then form QMC design sequences for
$H^{(d+1)/2}( \mathbb{S}^d )$. In the case, when $H^s(\mathbb{S}^d)$, with $d/2
< s < d/2 + 1$, is equipped with the reproducing kernel
$\KERNEL_{\mathrm{gd}}^{(s)}$ from \eqref{eq:K.gd.s}, a limiting process yields
that (cf.~\cite{BrWo2010Manuscript})
\begin{equation*}
\lim_{s \to (d/2)^+} \frac{\left[ \WCE_{H^s}(X_{N}) \right]^2 - 
\frac{1}{N}}{2s-d} = 
\frac{1}{N^2} \mathop{\sum_{i=1}^N \sum_{j=1}^N}_{i \neq j} 
\log \frac{1}{\left\| \PT{x}_i - \PT{x}_j \right\|} -  
V_{\mathrm{log}}( \mathbb{S}^d )
\end{equation*} 
for any $N$-point set $X_N = \{ \PT{x}_1, \dots, \PT{x}_N \} \subset
\mathbb{S}^d$. This suggests that the function space $H^{d/2}( \mathbb{S}^d )$
(which is not a reproducing kernel Hilbert space as it cannot be continuously
embedded into the space of continuous functions) is associated with the
logarithmic kernel, in a natural way. In that sense the logarithmic energy of
an $N$-point set can be understood as a limit of worst-case errors.

Stolarsky's invariance principle (cf. \cite{Stolarsky1973:sums_distances_ii}
and \cite{Brauchart_Dick2013:stolarskys_invariance}) states that the sum of all
mutual distances (a Riesz energy with Riesz parameter $-1$) and the spherical
cap $L^2$-discrepancy
\begin{equation*}
D_{L^2}(X_{N}) \DEF \left( \int_{0}^{\pi} \int_{\mathbb{S}^{d}} 
\left| \frac{1}{N}\sum_{\PT{y}\in X_N}\mathbbm{1}_{\PT{x}\in
    C(\PT{y},\theta)} - \sigma_d(C({\PT z}; \theta)) \right|^{2}
\dd{\sigma_d}({\PT z})\, \sin \theta \dd{\theta}\right)^{1/2}
\end{equation*}
is constant regardless of the choice of the node set $X_N$ on
$\mathbb{S}^d$. This principle connects in a very direct way the three areas
optimal energy (maximising the sum of distances), uniform distribution
(spherical cap $L^2$-discrepancy) and numerical integration (interpretation of
the double integral minus the double sum as worst-case error for functions in
$H^{(d+1)/2}( \mathbb{S}^d )$ provided with the distance kernel); i.e.,
\begin{equation*}
\frac{1}{N^2} \sum_{i=1}^N\sum_{j=1}^{N} \left\| \PT{x}_i - \PT{x}_j \right\| + 
\frac{1}{C_d} \left[ D_{L^2}(X_{N}) \right]^{2} = 
\int_{\mathbb{S}^d} \int_{\mathbb{S}^d} \left\| \PT{x}-\PT{y}\right\| 
\dd \sigma_d(\PT{x}) \,\dd \sigma_d(\PT{y}).
\end{equation*}
Furthermore, it provides a convenient way of computing the discrepancy
$D_{L^2}(X_{N})$ and it shows that for the particular setting of numerical
integration the spherical cap $L^2$-discrepancy is a constant multiple of the
worst-case error.
% where the spherical cap $L^2$-discrepancy is given by 
% \begin{equation*}
% D_{L^2}(X_{N}) \DEF \left( \int_{0}^{\pi} \int_{\mathbb{S}^{d}} \left| 
%\frac{1}{N}\sum_{\PT{y}\in X_N}\mathbbm{1}_{\PT{x}\in
%     C(\PT{y},\theta)} - \sigma_d(C({\PT z}; \theta)) \right|^{2}
%\dd{\sigma_d}({\PT z})\, \sin \theta \dd{\theta}\right)^{1/2}.
% \end{equation*}
The paper \cite{Brauchart_Dick2013:characterization_sobolev_spaces} gives an
extension of this principle to general powers of the distance (risen to the
power $2s-d$) involving the generalised spherical $L_2$-discrepancy
\begin{equation*}
\int_{0}^\pi \int_{\mathbb{S}^d} \left| \Delta_{X_N, \beta}(\PT{z}; \cos\theta) 
\right|^2 \dd \sigma_d( \PT{z} ) \sin \theta \dd \theta,
\end{equation*}
for the local discrepancy function (with smoothness index $s=\beta+(d-1)/2$)
\begin{equation*}
\Delta_{X_N, \beta}(\PT{z}; t) \DEF 
\frac{1}{N} \sum_{\PT{x} \in X_N} (\PT{x} \cdot \PT{z} - t)_+^{\beta-1} - 
\int_{\mathbb{S}^d} (\PT{y} \cdot \PT{z} - t)_+^{\beta-1} \,\dd \sigma_d(\PT{y}).
\end{equation*}
The paper~\cite{Grabner2014:point_minimal_energy} discusses further connections
between energy and discrepancy.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Main"
%%% End: 

